Security Analysis and Enhancement of Model Compressed Deep Learning Systems under Adversarial Attacks

DNN is presenting human-level performance for many complex intelligent tasks in real-world applications. However, it also introduces ever-increasing security concerns. For example, the emerging adversarial attacks indicate that even very small and often imperceptible adversarial input perturbations can easily mislead the cognitive function of deep learning systems (DLS). Existing DNN adversarial studies are narrowly performed on the ideal software-level DNN models with a focus on single uncertainty factor, i.e. input perturbations, however, the impact of DNN model reshaping on adversarial attacks, which is introduced by various hardware-favorable techniques such as hash-based weight compression during modern DNN hardware implementation, has never been discussed. In this work, we for the first time investigate the multi-factor adversarial attack problem in practical model optimized deep learning systems by jointly considering the DNN model-reshaping (e.g. HashNet based deep compression) and the input perturbations. We first augment adversarial example generating method dedicated to the compressed DNN models by incorporating the software-based approaches and mathematical modeled DNN reshaping. We then conduct a comprehensive robustness and vulnerability analysis of deep compressed DNN models under derived adversarial attacks. A defense technique named "gradient inhibition" is further developed to ease the generating of adversarial examples thus to effectively mitigate adversarial attacks towards both software and hardware-oriented DNNs. Simulation results show that "gradient inhibition" can decrease the average success rate of adversarial attacks from 87.99% to 4.77% (from 86.74% to 4.64%) on MNIST (CIFAR-10) benchmark with marginal accuracy degradation across various DNNs.

==> formula.tex <==

Cross-entropy loss function
\begin{equation}
J(x_i,t_j) = -\sum_{j=1}^n t_j \log F(z_j) 
\end{equation}





\begin{equation}
\label{hashae}
\begin{cases}
X^{AE} = X + \epsilon sgn(\nabla_XJ)\\
\nabla_XJ = \sum_{i=1}^{n^{l=2}} w_{h^{l=1}(i,j)}^{l=1} \xi^{l=1}(i,j)\delta_j^{l=2}\\
\delta_j^l=\left( \sum_{i=1}^{n^{l+1}} w_{h^{l}(i,j)}^l \xi^l(i,j)\delta_j^{l+1} \right)f^{'}(z_j^l)
\end{cases}
\end{equation}

==> outline.tex <==
\section{Outline}


Title--

%Security and robustness analysis of deep learning systems for adversarial attacks

Security Analysis and Enhancement of Model Compressed Deep Learning Systems under Adversarial Attacks

Author: Qi Liu, Tao Liu, Zihao Liu, Yanzhi Wang, Yier Jin, Wujie Wen

Abstract--
The state-of-the-art of Deep Neural Network (DNN) presents human-level performance on many complex intelligent tasks along with machine learning model innovation and recent hardware advancement.
%The recent impressive hardware advancement is demonstrating unsurpassed acceleration of deploying, 
However, it also introduces ever-increasing security concerns for those intelligent systems. For example, the emerging adversarial attacks, indicate that even small input imperceptible perturbation may severely destroy the cognitive functionality of deep learning systems (DLS). Although many relevant researches are conducted, all the existing DNN adversarial studies are based on the single uncertainty factor, i.e. input perturbations, and are solely performed on ideal software-level DNN models without considering DNN model reshaping introduced by various hardware-favorable techniques such as network pruning and HashNet during practical task executions in DNN hardware platforms. Whether and how those software-based attacks and defense solutions can be exerted and/or exploited in practical DLSs remain unexplored. In this work, we for the first time investigate the multi-factor adversarial attack problem in more practical hardware-oriented deep learning systems by jointly considering the DNN model-reshaping (e.g. HashNet based deep compression) and the input perturbations. 
%in the DNN model-reshaped practical deep learning systems by integrating highly compressed weights with input perturbations.
%the reshaped model has been characterized to develop the multi-factors adversarial attacks in deep learning systems by integrating highly compressed weights with input perturbations. 
Comprehensive robustness and vulnerability analysis are conducted based on the proposed semi-analytical modeling and simulation. %the proposed multi-factors adversarial attacks. 
Inspired from the security analysis, a defense technique named ``gradient inhibition" is further proposed to prevent the generating of input perturbations thus to effectively mitigate adversarial attacks towards either hardware oriented deep learning systems or software based DNNs. Simulation results well validate our proposed solution.

%However, the expensive computation and massive storage requirement significantly hinder its applications on resource limited platform. 
%The hardware-oriented Deep Learning System (DLS) become a promising solution for low-power, high-speed data processing greatly enriches intelligent applications. 

%Recently, security issues like adversarial attacks draw increasing attentions in DNN researches. Even inappreciable small input perturbations may severely destroy the cognitive functionality. 

%Unfortunately, the insidious security concerns have never been addressed in hardware designs, exposing serious threats to DLSs, thus urgently requirements of security analysis on vulnerabilities. However, all the existing DNN adversarial studies are based on the single uncertainty factor, i.e. input perturbations, and are solely performed on ideal software-level DNN models without considering the unique model reshaping during practical executions in DLS.

%Whether and how those software-based attacks and defense solutions can be exerted and/or exploited in practical DLSs remain unexplored.% and deserve thorough investigations.

%Our experimental results show that by adopting ``gradient inhibition'', the success rate of adversarial attacks has been reduced remarkably from 95.81\% to 0.22\% on MNIST benchmark.

Introduction--

1. DNNs show human-level performance on complex cognitive tasks, computer vision etc. However expensive computation and massive storage hinder applications on resource limited platform.

2. Hardware oriented deep learning systems become a promising solution offering low-power, high-speed hardware-based data processing which significantly enriches intelligent applications. Scalability has been greatly extended through model reshaping introduced by various hardware-favorable techniques.

3. Recently, security issues such as adversarial attacks are drawing increasing attentions in DNN researches. Through the intentionally perpetuated adversarial inputs, the cognitive functionality of DNNs can be severely destroyed.

4. Though deep learning systems are widely adopted in real-word applications, the insidious security concerns have never been addressed in existing researches, exposing serious threats to the robustness of deep learning systems, thus urgently requirements of security analysis on vulnerabilities in hardware-based deep learning systems.

5. However, all the existing DNN adversarial studies are based on the single uncertainty factor, i.e. input perturbations, and are solely performed on ideal software-level DNN models without considering the model reshaping during practical executions in deep learning systems. Whether and how those software-based attacks and defense solutions can be exerted and/or exploited in practical deep learning systems remain unexplored.% and deserve thorough investigations.

6. In this work, the reshaped model has been characterized to develop the multi-factors adversarial attacks in deep learning systems by integrating highly compressed weights with input perturbations. Robustness and vulnerabilities are measured by sandboxing the proposed multi-factors adversarial attacks. Inspired from the security analysis, a defense technique--``gradient inhibition'' is further proposed to prevent the generating of input perturbations thus effective mitigation on adversarial attacks for either hardware oriented deep learning systems or software based DNNs. Our experimental results show that by adopting ``gradient inhibition'', the success rate of adversarial attacks has been reduced remarkably from 95.81\% to 0.22\% on MNIST benchmark.

%the security and robustness analysis on deep learning systems is non-trivial due to the particularly compressed neural model. On one hand, the Adversarial


%More and more applications based on deep learning are widely used on devices with limited resources, such as mobile phones, which make hardware-deep learning system widely used, such as hashedNet.Recent research shows that deep learning is difficult to robust an attack called adversarial example that added a carefully selected small perturbation to the inputs.This makes us concern about security of deep learning system,whether they are vulnerable
%to adversarial example.we found that adversarial examples can misclassified by deep learning system,but their robustness to adversarial higher than uncompressed model.In this work,we focus on robustness of deep learning system to adversarial examples.

%An important idea to design compressed systems is to compress the number of parameters to reduce storage space,so that the system can be stored on devices with limited resources.thereby distribution of the parameters in the compressed system would be different with the uncompressed system.

Major Contributions:

1.we take the crafted adversarial example from soft-level to the hard-level.we study how to craft adversarial examples in the deep learning system.we found that robustness to adversarial higher than uncompressed model,and explains why the seemingly more vulnerable hardware-compressed model(like HashedNet) is better than the uncompressed model in robustness to adversarial example.
we will explain that how variation
of |w| impact crafting the AE.


2.inspired by the compressed system,we propose a defense technology to adversarial example.this simple and valid method greatly reduces the success rate of crafting adversarial sample(FGSM  AE crafting method from 95.81\% to 4.67\% ,and JSMA AE crafting method from 94.22\% to 0.22\% on MNIST dataset).

related work

Explaining and Harnessing Adversarial Examples[1]
Distillation as a Defense to Adversarial Perturbations against Deep Neural Networks[2]
TOWARDS DEEP NEURAL NETWORK ARCHITECTURES ROBUST TO ADVERSARIAL EXAMPLES[3]
Parseval Networks: Improving Robustness to Adversarial Examples[4]

almost robustness methods to AE
1 need to retrain network(用AE和clean example混合训练[1],改动了softmax，把用新的softmax训练好的模型的输出（分类概率估计）搬到需要抵抗AE的网络再训练[2])
2 Need change network structure[3][4],then training(Previous work considered the problem of
constructing such defenses but solutions proposed are deficient
in that they require making modifications to the DNN
architecture or only partially prevent adversarial samples from
being effective（[2]作者原话）)
Those methods have high time cost,or performance decrease
我们的方法不需要重新训练，没有结构上的改变，只是在训练好的模型上做处理，做到0 cost to robust AE
主要突出要rubust AE是很复杂，很难，很多人在work，就算有些加强了robustness但cost高，我们的方法简单有效，cost还小
我们发现越deep的网络，越容易被攻击（success rate 高），我们的方法反而能让它们更具robustness，描述VGG,googleNet层数都很多
Prelim
1.deep learning system:hashedNet
why compress
how to compress
2.how to craft AE in soft-level
FGSM(fast gradient sign method)
JSMA(Jacobian-based Saliency Map Approach)



our work
1.exploration to robustness to AE in hardware-level 
1.1:how combine AE in software-level with deep learning system together and show AE success rate result in the hashedNet.
1.2.
1.2.1 using crafting AE method formulas to demonstrate that different |w| can impact crafting the AE
1.2.2 |w| in the hashedNet is different with uncompressed system
how different
why different
different |w| how to impact AE.
|w| increase , adversarial gradient decrease(sensitivity to inputs decrease),so that difficult to craft AE.

2.defense technology to AE
We propose a new method to add the small perturbation in the weight to defense against adversarial examples. This perturbation is in the same direction as the weight.
why work
The result in MNIST (FGSM,JSMA)
Robustness Analysis 

Eval
CIFAR10(FGSM and JSMA)






Con






	
    

\section{Related Work}


contribution:

1.We found that the adversarial example black-box attack effect of the hardware-compressed model is weaker than uncompressed model.Although their respective AE can effectively attack themselves, they are not robust to its own adversarial examples.In other words, the compressed model can craft AE that appears to be capable of attack, but this kind of adversarial examples can't transfer to uncompressed models and attack uncompressed model  effectively.

2.the hardware-compressed model, their weights have different distributions and characteristics compared with uncompressed models after training convergence.We will discuss the effect of the change of weight on the Transferable rate of adversarial examples and  the robustness of model to adversarial examples.

3.We will propose a new method to decrease the adversarial examples Transferability further.

\section{HashedNet and Adversarial examples}

\subsection{HashedNet}
\subsection{Adversarial examples}




\section{Transferability of deep compression neural network black-box attacks using adversarial sample}

\subsection{The weight distribution features of hardware-compressed model}
   Some deep compression neural network model, such as using hash technology compressed model,After the model training converges, the probability distribution of weights is very different from the uncompressed model , even if their weights have the same initial value(Figure~\ref{fig:inital_weight_trained_weight_nn_hash}).
    
    
\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{inital_weight_trained_weight_nn_hash.png}
\caption{\label{fig:inital_weight_trained_weight_nn_hash}The neural network structure and the training parameters are exactly the same as the compressed model and the uncompressed model. Even if their weight value has the same initial value, after the model training converges,the solution region in weight space is different,in general, and the weight of The compressed mode has a larger first-order norm of mean and variance than uncompressed model}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{nn_hash_weight_distribution.png}
\caption{\label{fig:nn_hash_weight_distribution}After the model of training convergence, uncompressed model and compression model of weight distribution is different, the left is uncompressed model, the weight distribution is more concentrated and smooth, on the right is the compressed model, the weight distribution is flat and rough}
\end{figure}

\begin{table}
\centering
\begin{tabular}{l|r|r|r}
model type & uncompressed model & hashed compressed model \\\hline
mean(|weight|) &  0.0223 & 0.1911\\
variance(weight) & 8.3748e-04 & 0.0571 
\end{tabular}
\caption{\label{tab:The mean and variance}The mean and variance of the first order norm of the weight in uncompressed model and compressed model}
\end{table}

The weight of hashedNet is based on weight sharing.The real weight is stored in a hash bucket,which has provide values for virtual weights.There is an index table between real weight and virtual weight values to store their mapping relationships.the real weights is updated with the back-propagation algorithm instead of virtual weight.In general, the weight distribution of the compressed model is more flat and rough than uncompressed model(Figure ~\ref{fig:nn_hash_weight_distribution}), which means that the first-order norm of mean and variance of weight will increase(Table ~\ref{tab:The mean and variance}).
h


The main reason for this phenomenon is that after the weight sharing.As the valid weight decreases, each weight in the compressed model is more important than the uncompressed model.As we know, the more important a weight in a model, the greater its first-order norm.The higher the compression ratio, the greater the weight gain.generally, the common model with convolution layers and fully connected layers, whether or not the weight of model is compressed, the weights’ first-order norm in the first layer of convolution layers and last layer of the fully connected layers will be bigger than the other layer. the reason is that the number of valid weight in the first  layer and last layer less than other layer.

	The experiment shows that the distribution characteristics of the weight will affect the success rate of the attack of adversarial example crafted by hashed compressed model.
First, the attacker needs to craft adversarial example on his own model and then use it to attack the model he made, known as white box attack.If white-box attacks get a higher success rate, based on the theory of adversarial example attacks with transferability, this attack is also effective for other models, even if we don't know  the threatened model's structure and parameters, the so-called black-box attack.

\subsection{white-box attack using adversarial example in compressed model}
adversarial example white box attack refers to our known opponent structure and parameters, crafting adversarial example to attack the opponent.In our experiment, we used the exact same structure, the same training parameters, in the compression model and the uncompressed model.The dataset is using mnist .We control the compression ratio of hashed compressed model, so that the error rate of test is similar to that of uncompressed model.We found that the compressed model and uncompressed model showed similar vulnerability in the face of adversarial example white-box attack.

 respectively, the use of FGSM, compression attack success rate is slightly lower than uncompressed model(Figure ~\ref{fig:FGSM_write_box_attack_success_rate}) (epsilon is equal to 0.3, Success rate difference is 16\% ), use JSMA, compression model success rate is slightly higher than uncompressed model attack(Figure ~\ref{fig:JSMA_write_box_attack_success_rate}) (gamma is equal to 15\%, difference is 21\% ).
	



	


\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{FGSM_write_box_attack_success_rate.png}
\caption{\label{fig:FGSM_write_box_attack_success_rate}Using FGSM  adversarial example  algorithm to craft AE in compression model and uncompressed model to attack their own models separately.}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{JSMA_write_box_attack_success_rate.png}
\caption{\label{fig:JSMA_write_box_attack_success_rate}Using JSMA  adversarial example  algorithm to craft AE in compression model and uncompressed model to attack their own models separately.}
\end{figure}

\subsection{black-box attack using adversarial example}
The research shows that adversarial example has the transferability. It means that Adversarial examples are crafted using the DNN attacker model are not only misclassified
by the attacker model but also by the other DNN.
We found that the increase of first-order norm of weight will decrease even block adversarial example transfer to other model .the adversarial example crafted by compressed model can achieve a higher success rate on its own ,but The attacking effect of these  adversarial example on other models is not obvious.in black-box attack situation,we don't know structure of defense model.


We know that most attacks are based on black-box attacks, and there are cracker who use publicly available models to craft adversarial example to attack other models.Blocking the model's adversarial example transferability means that these models are not easily exploited by crackers to attack other models

We can compare the transferability of the compression model and the uncompressed model.uncompressed model as an attacker,using the adversarial example craft by FGSM in uncompressed model to attack other models, when epsilon is equal to 0.3,The average success rate was from 76.53\% to 57.54\%.In other words, an average of 75.19\% of adversarial example successfully transfer from the attacker model(Figure ~\ref{fig:FGSM_nn_anymodel_transferability}).However,if compressed model acted as an attacker,when epsilon is equal to 0.3,The average success rate was from 60.22\% to 17.53\%.(an average of 29.11\% of adversarial example successfully transfer from the attacker model).


In the experiment we also found some interesting phenomena, we was discussing just now are all the uncompressed model or compressed as the attacker, and model of our attack is a black box, to compare their adversarial example transferability success rate.Now changing the position, the attacker as a black-box,while uncompressed model or the compressed model acted as defenders, we found that The compressed model is a little stronger than the uncompressed model resist adversarial example(Figure ~\ref{fig:nn_hash_defense_AE}).In experience, the compressed model with the accuracy or number of weight loss, should be more difficult to resist adversarial example.





The weight distribution of the compressed model is flat and the first-order norm of the weight is larger than uncompressed model. So that adversarial example crafted by compressed model is difficult to attack other model, It means the decrease of the transferability success rate of adversarial example.



	
\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{FGSM_nn_anymodel_transferability.png}
\caption{\label{fig:FGSM_nn_anymodel_transferability}adversarial example  crafted in the uncompressed model transfer to other model.}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{FGSM_hash_anymodel_transferability.png}
\caption{\label{fig:FGSM_hash_anymodel_transferability}adversarial example  crafted in the hashed compressed model transfer to other model.}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{nn_hash_defense_AE.png}
\caption{\label{fig:nn_hash_defense_AE}defense adversarial example in uncompressed model and hashed compressed model}
\end{figure}


There are two reasons for the decrease adversarial example transferability success rate of the compression model 
\subsubsection{impact of decision boundaries}

we know that adversarial examples are crafted using the DNN model are not only misclassified
by the attacker model but also by the other DNN,because both
models have similar decision boundaries.More precisely,When we craft a perturbation in the input data, the input moves in any direction to cross the decision boundaries,
this distance
traveled crossing a model’s decision boundary is on average larger than the distance separating
the decision boundaries of two models in that direction(Figure ~\ref{fig:nn_attack_DB}).Thus, adversarial perturbations are very likely to
transfer to other models with different architectures.

We know that if too large weight  can cause the curvature of the decision boundaries to rise,and the decision boundaries is closer to the data point, leading to overfiting.
firstly,We need to explain that the hashed compression model has not overfitting. Using the mnist dataset, it has an error rate of 0.9\% in the test stage, while the uncompressed model is 0.7\% in our experiment.

but there is a tendency for decision boundaries to be close to data points.So we can predict that,when the input moves in adversarial examples attack direction to cross the decision boundaries, adversarial examples attack region craft by attacker model is between the decision boundaries of two models in adversarial examples attack direction.in Figure ~\ref{fig:nn_hash_attack_DB2},we can see that the adversarial examples crafted by hashed compressed are misclassified by the itself,but it can't be misclassified by the uncompressed model.





\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{nn_attack_DB.png}
\caption{\label{fig:nn_attack_DB}decision boundaries of two uncompressed model.}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{nn_hash_attack_DB2.png}
\caption{\label{fig:nn_hash_attack_DB2}decision boundaries of uncompressed model and hashed compressed model}
\end{figure}


\subsubsection{impact of  sensitivity to inputs}

Another important reason is that the hashed compression model is less sensitive to input changes than uncompressed model.

 output of the linear model can be broadly as such a function 
 \begin{equation}
  F (x) = wx+b
 \end{equation}


 if we add the any kind of perturbation on the input, we can write this function

 \begin{equation}
  F (x+\triangle x) =w*x+ w * \triangle x+b
 \end{equation} 
 is perturbation to output.

intuitively,the larger first order of weight , the greater the perturbation to the output. It means that same perturbation makes the compressed classifier fooled easier.but if this perturbation is adversarial noise,The situation will be more complicated.

Whether FGSM or JSMA adversarial example crafting method, they are based on the gradient.
Let $\theta$ be the parameters of a model, x the input to the model, t is the target class(the value is 1 or 0),F(x) the output of model and J($\theta$, x, t) be the cost function.
They calculate separately $
\triangledown _x J( \theta ,x ,t )$ and $
\triangledown _x F( \theta ,x) $.
 hashed compressed model can reduce gradients exploited by adversaries to craft perturbations. This means that it is insensitive to the input of adversarial example perturbations.
 
Let me give you a simple example to explain it.Let us
consider the neural network with two layers.the output layer uses the softmax function, and the loss function use the cross entropy error function.We assume the  weights second layer w(In the hashed compressed model we use virtual weight to calculate the gradient, which is consistent with the uncompressed model).The output before entering the softmax function is
  \begin{equation}
 z_j=\sum_{i=1}^n w_{ji}x_i
 \end{equation}
 so softmax function is 
   \begin{equation}
F(z_j)=\frac{e^{z_j}}{\sum_{k=1}^n e^{z_k}}
 \end{equation}
We can do some calculation to get the following equation
 \begin{equation}
\triangledown _{x_i} J( \theta ,x_i , t_j ) = \sum_{j=1}^n w_{ji}(F(z_j)-t_j)
 \end{equation}
 We can easily found, when we increased first norm of weight,$F(z_j)$ or closer 1 ( have higher confidence for j class), or closer 0 (confidence reduce for other class), which makes the $(F(z_j)-t_j)$ closer 0.there are  smaller gradient in the compressed model.It's also important to note that  weight is increasing in the final calculation (5) ,but it's trivial to be $(F(z_j)-t_j)$ closer to 0.
 
 we evaluate the mean amplitude of these gradients on hashed compressed models and uncompressed model in(figure ~\ref{fig:FGSM_gradient_nn_hash}).
 
Same thing in computing $
\triangledown F( \theta ,x) $ in the JSMA.
 \begin{equation}
\triangledown _{x_i} F( \theta ,x_i) = \sum_{j=1}^n w_{ji}F(z_j)(1-F(z_j))
 \end{equation}

\subsection{ new method to further decrease the adversarial examples Transferability }

To Magnify the phenomenon, we use a new method to increase the first-order norm of weights.

 \begin{equation}
w = w + \tau * sign (w)
 \end{equation}
 
This method is used in test stage.the error rate is almost the same as before in mnist dataset((Table ~\ref{tab:error rate new method})). in the figure ~\ref{fig:FGSM_gradient_new_method},we can see the mean amplitude of  gradients using this method.Using the new method can reduce the migration of the model better(figure ~\ref{fig:new_method_transferability})

 

\begin{table}
\centering
\begin{tabular}{l|r|r|r|r}
$\tau$ & 0 & 0.01& 0.02&0.05 \\\hline
error rate &  0.7\% & 0.79\% & 0.82\% & 0.89\% \\
 
\end{tabular}
\caption{\label{tab:error rate new method}error rate}
\end{table}





\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{FGSM_gradient_nn_hash.png}
\caption{\label{fig:FGSM_gradient_nn_hash}mean amplitude of these gradients on hashed compressed models and uncompressed model.}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{FGSM_gradient_new_method.png}
\caption{\label{fig:FGSM_gradient_new_method}mean amplitude of these gradients on new model.}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{new_method_transferability.png}
\caption{\label{fig:new_method_transferability}transferability in the new model.}
\end{figure}



\section{Experiment}

We apply this method to the cifar10 data set, and the same result is obtained. We first use the weight increment method on the previously trained  model(attacker model), then using this model to craft adversarial example , and use it to attack defender model to see if AE can transfer to the defender model.

We found,With the increase of the first order norm of weights, the transferability of the adversarial example decreases dramatically(figure ~\ref{fig:new_method_transferability}), while the error rate of the test increases by only about 2\%.

\begin{table}
\centering
\begin{tabular}{l|r|r|r|r}
structure&attacker model &  DNN1 & DNN2&  DNN3 \\\hline
convolution layer& 4 layers  &  3 layers & 6 layers & 9 layers \\\hline
fully connected layer& 2 layers  &  1 layers & 2 layers & 2 layers \\\hline
activation function& relu  &  relu & tanh & relu \\\hline

output layer function& softmax  &  softmax & softmax & softmax \\\hline
 
\end{tabular}
\caption{\label{tab:error rate new method}error rate}
\end{table}

To ensure the accuracy of the model, we only use this method on the two layer fully connected layer of the model.


\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{new_method_transferability_cifar10.png}
\caption{\label{fig:new_method_transferability_cifar10}transferability in the new model.}
\end{figure}





	
    

\section{Related Work}


contribution:

1.We found that the adversarial example black-box attack effect of the hardware-compressed model is weaker than uncompressed model.Although their respective AE can effectively attack themselves, they are not robust to its own adversarial examples.In other words, the compressed model can craft AE that appears to be capable of attack, but this kind of adversarial examples can't transfer to uncompressed models and attack uncompressed model  effectively.

2.the hardware-compressed model, their weights have different distributions and characteristics compared with uncompressed models after training convergence.We will discuss the effect of the change of weight on the Transferable rate of adversarial examples and  the robustness of model to adversarial examples.

3.We will propose a new method to decrease the adversarial examples Transferability further.

\section{HashedNet and Adversarial examples}

\subsection{HashedNet}
\subsection{Adversarial examples}




\section{Transferability of deep compression neural network black-box attacks using adversarial sample}

\subsection{The weight distribution features of hardware-compressed model}
   Some deep compression neural network model, such as using hash technology compressed model,After the model training converges, the probability distribution of weights is very different from the uncompressed model , even if their weights have the same initial value(Figure~\ref{fig:inital_weight_trained_weight_nn_hash}).
    
    
\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{inital_weight_trained_weight_nn_hash.png}
\caption{\label{fig:inital_weight_trained_weight_nn_hash}The neural network structure and the training parameters are exactly the same as the compressed model and the uncompressed model. Even if their weight value has the same initial value, after the model training converges,the solution region in weight space is different,in general, and the weight of The compressed mode has a larger first-order norm of mean and variance than uncompressed model}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{nn_hash_weight_distribution.png}
\caption{\label{fig:nn_hash_weight_distribution}After the model of training convergence, uncompressed model and compression model of weight distribution is different, the left is uncompressed model, the weight distribution is more concentrated and smooth, on the right is the compressed model, the weight distribution is flat and rough}
\end{figure}

\begin{table}
\centering
\begin{tabular}{l|r|r|r}
model type & uncompressed model & hashed compressed model \\\hline
mean(|weight|) &  0.0223 & 0.1911\\
variance(weight) & 8.3748e-04 & 0.0571 
\end{tabular}
\caption{\label{tab:The mean and variance}The mean and variance of the first order norm of the weight in uncompressed model and compressed model}
\end{table}

The weight of hashedNet is based on weight sharing.The real weight is stored in a hash bucket,which has provide values for virtual weights.There is an index table between real weight and virtual weight values to store their mapping relationships.the real weights is updated with the back-propagation algorithm instead of virtual weight.In general, the weight distribution of the compressed model is more flat and rough than uncompressed model(Figure ~\ref{fig:nn_hash_weight_distribution}), which means that the first-order norm of mean and variance of weight will increase(Table ~\ref{tab:The mean and variance}).
h


The main reason for this phenomenon is that after the weight sharing.As the valid weight decreases, each weight in the compressed model is more important than the uncompressed model.As we know, the more important a weight in a model, the greater its first-order norm.The higher the compression ratio, the greater the weight gain.generally, the common model with convolution layers and fully connected layers, whether or not the weight of model is compressed, the weights’ first-order norm in the first layer of convolution layers and last layer of the fully connected layers will be bigger than the other layer. the reason is that the number of valid weight in the first  layer and last layer less than other layer.

	The experiment shows that the distribution characteristics of the weight will affect the success rate of the attack of adversarial example crafted by hashed compressed model.
First, the attacker needs to craft adversarial example on his own model and then use it to attack the model he made, known as white box attack.If white-box attacks get a higher success rate, based on the theory of adversarial example attacks with transferability, this attack is also effective for other models, even if we don't know  the threatened model's structure and parameters, the so-called black-box attack.

\subsection{white-box attack using adversarial example in compressed model}
adversarial example white box attack refers to our known opponent structure and parameters, crafting adversarial example to attack the opponent.In our experiment, we used the exact same structure, the same training parameters, in the compression model and the uncompressed model.The dataset is using mnist .We control the compression ratio of hashed compressed model, so that the error rate of test is similar to that of uncompressed model.We found that the compressed model and uncompressed model showed similar vulnerability in the face of adversarial example white-box attack.

 respectively, the use of FGSM, compression attack success rate is slightly lower than uncompressed model(Figure ~\ref{fig:FGSM_write_box_attack_success_rate}) (epsilon is equal to 0.3, Success rate difference is 16\% ), use JSMA, compression model success rate is slightly higher than uncompressed model attack(Figure ~\ref{fig:JSMA_write_box_attack_success_rate}) (gamma is equal to 15\%, difference is 21\% ).
	



	


\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{FGSM_write_box_attack_success_rate.png}
\caption{\label{fig:FGSM_write_box_attack_success_rate}Using FGSM  adversarial example  algorithm to craft AE in compression model and uncompressed model to attack their own models separately.}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{JSMA_write_box_attack_success_rate.png}
\caption{\label{fig:JSMA_write_box_attack_success_rate}Using JSMA  adversarial example  algorithm to craft AE in compression model and uncompressed model to attack their own models separately.}
\end{figure}

\subsection{black-box attack using adversarial example}
The research shows that adversarial example has the transferability. It means that Adversarial examples are crafted using the DNN attacker model are not only misclassified
by the attacker model but also by the other DNN.
We found that the increase of first-order norm of weight will decrease even block adversarial example transfer to other model .the adversarial example crafted by compressed model can achieve a higher success rate on its own ,but The attacking effect of these  adversarial example on other models is not obvious.in black-box attack situation,we don't know structure of defense model.


We know that most attacks are based on black-box attacks, and there are cracker who use publicly available models to craft adversarial example to attack other models.Blocking the model's adversarial example transferability means that these models are not easily exploited by crackers to attack other models

We can compare the transferability of the compression model and the uncompressed model.uncompressed model as an attacker,using the adversarial example craft by FGSM in uncompressed model to attack other models, when epsilon is equal to 0.3,The average success rate was from 76.53\% to 57.54\%.In other words, an average of 75.19\% of adversarial example successfully transfer from the attacker model(Figure ~\ref{fig:FGSM_nn_anymodel_transferability}).However,if compressed model acted as an attacker,when epsilon is equal to 0.3,The average success rate was from 60.22\% to 17.53\%.(an average of 29.11\% of adversarial example successfully transfer from the attacker model).


In the experiment we also found some interesting phenomena, we was discussing just now are all the uncompressed model or compressed as the attacker, and model of our attack is a black box, to compare their adversarial example transferability success rate.Now changing the position, the attacker as a black-box,while uncompressed model or the compressed model acted as defenders, we found that The compressed model is a little stronger than the uncompressed model resist adversarial example(Figure ~\ref{fig:nn_hash_defense_AE}).In experience, the compressed model with the accuracy or number of weight loss, should be more difficult to resist adversarial example.





The weight distribution of the compressed model is flat and the first-order norm of the weight is larger than uncompressed model. So that adversarial example crafted by compressed model is difficult to attack other model, It means the decrease of the transferability success rate of adversarial example.



	
\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{FGSM_nn_anymodel_transferability.png}
\caption{\label{fig:FGSM_nn_anymodel_transferability}adversarial example  crafted in the uncompressed model transfer to other model.}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{FGSM_hash_anymodel_transferability.png}
\caption{\label{fig:FGSM_hash_anymodel_transferability}adversarial example  crafted in the hashed compressed model transfer to other model.}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{nn_hash_defense_AE.png}
\caption{\label{fig:nn_hash_defense_AE}defense adversarial example in uncompressed model and hashed compressed model}
\end{figure}


There are two reasons for the decrease adversarial example transferability success rate of the compression model 
\subsubsection{impact of decision boundaries}

we know that adversarial examples are crafted using the DNN model are not only misclassified
by the attacker model but also by the other DNN,because both
models have similar decision boundaries.More precisely,When we craft a perturbation in the input data, the input moves in any direction to cross the decision boundaries,
this distance
traveled crossing a model’s decision boundary is on average larger than the distance separating
the decision boundaries of two models in that direction(Figure ~\ref{fig:nn_attack_DB}).Thus, adversarial perturbations are very likely to
transfer to other models with different architectures.

We know that if too large weight  can cause the curvature of the decision boundaries to rise,and the decision boundaries is closer to the data point, leading to overfiting.
firstly,We need to explain that the hashed compression model has not overfitting. Using the mnist dataset, it has an error rate of 0.9\% in the test stage, while the uncompressed model is 0.7\% in our experiment.

but there is a tendency for decision boundaries to be close to data points.So we can predict that,when the input moves in adversarial examples attack direction to cross the decision boundaries, adversarial examples attack region craft by attacker model is between the decision boundaries of two models in adversarial examples attack direction.in Figure ~\ref{fig:nn_hash_attack_DB2},we can see that the adversarial examples crafted by hashed compressed are misclassified by the itself,but it can't be misclassified by the uncompressed model.





\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{nn_attack_DB.png}
\caption{\label{fig:nn_attack_DB}decision boundaries of two uncompressed model.}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{nn_hash_attack_DB2.png}
\caption{\label{fig:nn_hash_attack_DB2}decision boundaries of uncompressed model and hashed compressed model}
\end{figure}


\subsubsection{impact of  sensitivity to inputs}

Another important reason is that the hashed compression model is less sensitive to input changes than uncompressed model.

 output of the linear model can be broadly as such a function 
 \begin{equation}
  F (x) = wx+b
 \end{equation}


 if we add the any kind of perturbation on the input, we can write this function

 \begin{equation}
  F (x+\triangle x) =w*x+ w * \triangle x+b
 \end{equation} 
 is perturbation to output.

intuitively,the larger first order of weight , the greater the perturbation to the output. It means that same perturbation makes the compressed classifier fooled easier.but if this perturbation is adversarial noise,The situation will be more complicated.

Whether FGSM or JSMA adversarial example crafting method, they are based on the gradient.
Let $\theta$ be the parameters of a model, x the input to the model, t is the target class(the value is 1 or 0),F(x) the output of model and J($\theta$, x, t) be the cost function.
They calculate separately $
\triangledown _x J( \theta ,x ,t )$ and $
\triangledown _x F( \theta ,x) $.
 hashed compressed model can reduce gradients exploited by adversaries to craft perturbations. This means that it is insensitive to the input of adversarial example perturbations.
 
Let me give you a simple example to explain it.Let us
consider the neural network with two layers.the output layer uses the softmax function, and the loss function use the cross entropy error function.We assume the  weights second layer w(In the hashed compressed model we use virtual weight to calculate the gradient, which is consistent with the uncompressed model).The output before entering the softmax function is
  \begin{equation}
 z_j=\sum_{i=1}^n w_{ji}x_i
 \end{equation}
 so softmax function is 
   \begin{equation}
F(z_j)=\frac{e^{z_j}}{\sum_{k=1}^n e^{z_k}}
 \end{equation}
We can do some calculation to get the following equation
 \begin{equation}
\triangledown _{x_i} J( \theta ,x_i , t_j ) = \sum_{j=1}^n w_{ji}(F(z_j)-t_j)
 \end{equation}
 We can easily found, when we increased first norm of weight,$F(z_j)$ or closer 1 ( have higher confidence for j class), or closer 0 (confidence reduce for other class), which makes the $(F(z_j)-t_j)$ closer 0.there are  smaller gradient in the compressed model.It's also important to note that  weight is increasing in the final calculation (5) ,but it's trivial to be $(F(z_j)-t_j)$ closer to 0.
 
 we evaluate the mean amplitude of these gradients on hashed compressed models and uncompressed model in(figure ~\ref{fig:FGSM_gradient_nn_hash}).
 
Same thing in computing $
\triangledown F( \theta ,x) $ in the JSMA.
 \begin{equation}
\triangledown _{x_i} F( \theta ,x_i) = \sum_{j=1}^n w_{ji}F(z_j)(1-F(z_j))
 \end{equation}

\subsection{ new method to further decrease the adversarial examples Transferability }

To Magnify the phenomenon, we use a new method to increase the first-order norm of weights.

 \begin{equation}
w = w + \tau * sign (w)
 \end{equation}
 
This method is used in test stage.the error rate is almost the same as before in mnist dataset((Table ~\ref{tab:error rate new method})). in the figure ~\ref{fig:FGSM_gradient_new_method},we can see the mean amplitude of  gradients using this method.Using the new method can reduce the migration of the model better(figure ~\ref{fig:new_method_transferability})

 

\begin{table}
\centering
\begin{tabular}{l|r|r|r|r}
$\tau$ & 0 & 0.01& 0.02&0.05 \\\hline
error rate &  0.7\% & 0.79\% & 0.82\% & 0.89\% \\
 
\end{tabular}
\caption{\label{tab:error rate new method}error rate}
\end{table}





\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{FGSM_gradient_nn_hash.png}
\caption{\label{fig:FGSM_gradient_nn_hash}mean amplitude of these gradients on hashed compressed models and uncompressed model.}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{FGSM_gradient_new_method.png}
\caption{\label{fig:FGSM_gradient_new_method}mean amplitude of these gradients on new model.}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{new_method_transferability.png}
\caption{\label{fig:new_method_transferability}transferability in the new model.}
\end{figure}



\section{Experiment}

We apply this method to the cifar10 data set, and the same result is obtained. We first use the weight increment method on the previously trained  model(attacker model), then using this model to craft adversarial example , and use it to attack defender model to see if AE can transfer to the defender model.

We found,With the increase of the first order norm of weights, the transferability of the adversarial example decreases dramatically(figure ~\ref{fig:new_method_transferability}), while the error rate of the test increases by only about 2\%.



To ensure the accuracy of the model, we only use this method on the two layer fully connected layer of the model.


\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{new_method_transferability_cifar10.png}
\caption{\label{fig:new_method_transferability_cifar10}transferability in the new model.}

\end{figure}










==> plot.tex <==

design
(outline our work 1.1)
描述hashedNet要比nn robustness好一些
图1.FGSM AE success rate in MNIST(epsilon 0.1-0.5)(nn,hash1/8,hash1/64)
图2.JSMA AE success rate in MNIST(gamma 0.05-0.15)(nn,hash1/8,hash1/64)

(outline our work 1.2.2)
分析原因，是因为amplitude of adversarial gradient小了
(down)图3.amplitude of adversarial gradient FGSM（nn,hash1/8,hash1/64）(之前在1.2.1描述了|W|如何影响gradient，这里只画FGSM的gradient)





(outline our work 2) defense
我们可以使用新的方法w=w+tsign(w),扩大|w|,缩小gradient，先在hash上用（注意说我们这个方法可以把gradient直接缩小成0（和Distillation不太一样，论文没说它能把gradient变为0），也就是说太小了，精度缺失，机器表示不了这么多位，从而彻底的阻止AE的攻击（rubostness to AE））
(down)图4 amplitude of adversarial gradient(用在hash1/8上)(t=0-0.1)



分析robustness，新方法是怎么一步步增加nn,hash的robustness的
图7 FGSM,JSMA robustness increase(nn,hash1/8)(t=0-0.1)



(outline experiment)

过渡到nn，我们发现在nn上也可以用，抵抗AE效果还更好，而且accuracy变化小
(down)图5 FGSM and JSMA success rate(nn,hash1/8) (t=0-0.1)
(down)图6 accuracy variation(nn,hash1/8)(t=0-0.1)

上面都都是以mnist为例子的讨论，现在要用到cifar10，更复杂的数据集,这里都讨论nn
1.我们发现越deep的网络，越容易被攻击（success rate 高），我们的方法反而能让它们更具robustness，
描述VGG,googleNet层数都很多我们使用VGG来训练cifar10
图8.DNN1,DNN2,DNN3,VGG FGSM success rate



2.选取那一层进行|w| increase 是一个问题，我们发现越接近output layer层（fully connected layer）accuracy下降越小，neural 越多的层（fully connected layer）对|w| increase的收益大，robustness增加明显
图9.accuracy variation 以DNN2为例，每一层用新方法
图10.FGSM success rate 以DNN2为例，每一层用新方法



performance evaluation 




==> setup.tex <==
你把用的model struture, database还有 epsilong这些参数先给我。我写experiment setup

dataset MNIST

model structure

convolution 2层
fully connected layer 1 层
output layer function: SoftMax
activation function:ReLU
loss function:Cross Entropy








==> table.tex <==
\begin{table}
\centering
\caption{\label{tab:accuracy baseline}accuracy baseline of selected neural network candidates.}
\begin{tabular}{|c|c|c|c|c|}
\hline
Candidate Models     & DNN1     & DNN2     & DNN3     & VGG-16 \\ \hline
Accuracy   & 79.63\% &86.35\% & 87\% & 92.1\%      \\ \hline

\end{tabular}
\end{table}
